INSIGHT: INference-time Sequence Introspection for Generating Help Triggers in Vision-Language-Action Models

Recent Vision-Language-Action (VLA) models show strong generalization capabilities, yet they lack introspective mechanisms for anticipating failures and requesting help from a human supervisor. We present \textbf{INSIGHT}, a learning framework for leveraging token-level uncertainty signals to predict when a VLA should request help. Using $\pi_0$-FAST as the underlying model, we extract per-token \emph{entropy}, \emph{log-probability}, and Dirichlet-based estimates of \emph{aleatoric and epistemic uncertainty}, and train compact transformer classifiers to map these sequences to help triggers. We explore supervision regimes for strong or weak supervision, and extensively compare them across in-distribution and out-of-distribution tasks. Our results show a trade-off: strong labels enable models to capture fine-grained uncertainty dynamics for reliable help detection, while weak labels, though noisier, still support competitive introspection when training and evaluation are aligned, offering a scalable path when dense annotation is impractical. Crucially, we find that modeling the temporal evolution of token-level uncertainty signals with transformers provides far greater predictive power than static sequence-level scores. This study provides the first systematic evaluation of uncertainty-based introspection in VLAs, opening future avenues for active learning and for real-time error mitigation through selective human intervention.

==> id_figures_old.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/ID/test_strong_accuracy_seaborn_grouped.png}
    \caption{}
    \label{fig:ID_strong_acc}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/ID/test_strong_f1_seaborn_grouped.png}
    \caption{}
    \label{fig:ID_strong_f1}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/ID/test_weak_accuracy_seaborn_grouped.png}
    \caption{}
    \label{fig:ID_weak_acc}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/ID/test_strong_f1_seaborn_grouped.png}
    \caption{}
    \label{fig:ID_weak_f1}
\end{figure}


==> lid_figures_old.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/LID/test_strong_accuracy_seaborn_grouped.png}
    \caption{}
    \label{fig:LID_strong_acc}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/LID/test_strong_f1_seaborn_grouped.png}
    \caption{}
    \label{fig:LID_strong_acc}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/LID/test_weak_accuracy_seaborn_grouped.png}
    \caption{}
    \label{fig:LID_weak_acc}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/LID/test_strong_f1_seaborn_grouped.png}
    \caption{}
    \label{fig:LID_weak_f1}
\end{figure}

==> ood_figures_old.tex <==

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/OOD/ood_test_strong_accuracy_seaborn.png}
    \caption{}
    \label{fig:OOD_strong_acc}
\end{figure}

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/OOD/ood_test_strong_f1_seaborn.png}
    \caption{}
    \label{fig:OOD_strong_f1}
\end{figure}

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/OOD/ood_test_weak_accuracy_seaborn.png}
    \caption{}
    \label{fig:OOD_weak_acc}
\end{figure}

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/OOD/ood_test_weak_f1_seaborn.png}
    \caption{}
    \label{fig:OOD_weak_f1}
\end{figure}

==> tables.tex <==
\subsection{In-Distribution Test Results}
Here we provide the detailed results of our in-distribution test results.
\begin{table*}[h]
\centering
\small
\begin{tabular}{lcccc}
\toprule
Method & Acc. & Prec. & Rec. & F1 \\
\midrule
Strong Superv. & \textbf{0.887 $\pm$ 0.044} & 0.800 $\pm$ 0.122 & 0.784 $\pm$ 0.102 & \textbf{0.782 $\pm$ 0.075} \\
Weak Superv. & 0.762 $\pm$ 0.091 & 0.853 $\pm$ 0.137 & 0.185 $\pm$ 0.102 & 0.288 $\pm$ 0.123 \\
CP-S (entropy) & 0.484 $\pm$ 0.034 & 0.323 $\pm$ 0.100 & 0.818 $\pm$ 0.090 & 0.450 $\pm$ 0.096 \\
CP-S (perplex) & 0.457 $\pm$ 0.042 & 0.311 $\pm$ 0.102 & 0.813 $\pm$ 0.094 & 0.438 $\pm$ 0.104 \\
CP-W (entropy) & 0.502 $\pm$ 0.030 & 0.324 $\pm$ 0.100 & 0.763 $\pm$ 0.098 & 0.442 $\pm$ 0.094 \\
CP-W (perplex) & 0.489 $\pm$ 0.031 & 0.314 $\pm$ 0.099 & 0.743 $\pm$ 0.087 & 0.430 $\pm$ 0.095 \\
\bottomrule
\end{tabular}
\vspace{3pt}
\caption{Help detection on \textbf{Test=STRONG} ($\beta=0.20$). Transformer shows mean$\pm$std over folds; CP shows entropy and perplexity (mean$\pm$std across folds).}
\label{tab:help_detection_test_strong_foldwise}
\end{table*}

\begin{table*}[h]
\centering
\small
\begin{tabular}{lcccc}
\toprule
Method & Acc. & Prec. & Rec. & F1 \\
\midrule
Strong Superv. & 0.756 $\pm$ 0.116 & 0.642 $\pm$ 0.196 & 0.957 $\pm$ 0.072 & \textbf{0.752 $\pm$ 0.150} \\
Weak Superv. & \textbf{0.812 $\pm$ 0.106} & 0.849 $\pm$ 0.168 & 0.733 $\pm$ 0.233 & \textbf{0.751 $\pm$ 0.126} \\
CP-S (entropy) & 0.450 $\pm$ 0.174 & 0.450 $\pm$ 0.174 & 1.000 $\pm$ 0.000 & 0.603 $\pm$ 0.167 \\
CP-S (perplex) & 0.450 $\pm$ 0.174 & 0.450 $\pm$ 0.174 & 1.000 $\pm$ 0.000 & 0.603 $\pm$ 0.167 \\
CP-W (entropy) & 0.738 $\pm$ 0.121 & 0.677 $\pm$ 0.149 & 0.774 $\pm$ 0.147 & 0.710 $\pm$ 0.111 \\
CP-W (perplex) & 0.650 $\pm$ 0.122 & 0.549 $\pm$ 0.211 & 0.751 $\pm$ 0.165 & 0.628 $\pm$ 0.194 \\
\bottomrule
\end{tabular}
\vspace{3pt}
\caption{Help detection on \textbf{Test=WEAK} ($\beta=0.20$). Transformer shows mean$\pm$std over folds; CP shows entropy and perplexity (mean$\pm$std across folds).}
\label{tab:help_detection_test_weak_foldwise}
\end{table*}

\subsection{Distribution Shift Test Results}
Here we provide the detailed results of our distribution shift test results.

\begin{table*}[h]
\centering
\small
\begin{tabular}{lcccc}
\toprule
Method & Acc. & Prec. & Rec. & F1 \\
\midrule
Strong Superv. & \textbf{0.686 $\pm$ 0.036} & 0.728 $\pm$ 0.067 & 0.427 $\pm$ 0.104 & 0.532 $\pm$ 0.101 \\
Weak Superv. & 0.592 $\pm$ 0.026 & 0.705 $\pm$ 0.082 & 0.096 $\pm$ 0.031 & 0.167 $\pm$ 0.049 \\
CP-S (entropy) & 0.499 $\pm$ 0.022 & 0.451 $\pm$ 0.033 & 0.748 $\pm$ 0.043 & 0.562 $\pm$ 0.030 \\
CP-S (perplex) & 0.490 $\pm$ 0.023 & 0.446 $\pm$ 0.034 & 0.762 $\pm$ 0.040 & 0.562 $\pm$ 0.031 \\
CP-W (entropy) & 0.575 $\pm$ 0.025 & 0.532 $\pm$ 0.076 & 0.097 $\pm$ 0.026 & 0.163 $\pm$ 0.040 \\
CP-W (perplex) & 0.567 $\pm$ 0.027 & 0.490 $\pm$ 0.100 & 0.098 $\pm$ 0.019 & 0.162 $\pm$ 0.030 \\
\bottomrule
\end{tabular}
\vspace{3pt}
\caption{\textbf{DS} help-detection on \textbf{Test=STRONG}. Transformer shows mean$\pm$std over folds; CP shows entropy and perplexity (mean$\pm$std across folds).}
\label{tab:ood_help_detection_test_strong_foldwise}
\end{table*}

\begin{table*}[h]
\centering
\small
\begin{tabular}{lcccc}
\toprule
Method & Acc. & Prec. & Rec. & F1 \\
\midrule
Strong Superv. & \textbf{0.751 $\pm$ 0.052} & 0.753 $\pm$ 0.054 & 0.909 $\pm$ 0.080 & \textbf{0.821 $\pm$ 0.038} \\
Weak Superv. & 0.670 $\pm$ 0.062 & 0.854 $\pm$ 0.072 & 0.586 $\pm$ 0.116 & 0.686 $\pm$ 0.081 \\
CP-S (entropy) & 0.631 $\pm$ 0.041 & 0.631 $\pm$ 0.041 & 1.000 $\pm$ 0.000 & 0.773 $\pm$ 0.031 \\
CP-S (perplex) & 0.631 $\pm$ 0.041 & 0.631 $\pm$ 0.041 & 1.000 $\pm$ 0.000 & 0.773 $\pm$ 0.031 \\
CP-W (entropy) & 0.590 $\pm$ 0.065 & 0.682 $\pm$ 0.072 & 0.665 $\pm$ 0.040 & 0.672 $\pm$ 0.050 \\
CP-W (perplex) & 0.644 $\pm$ 0.065 & 0.717 $\pm$ 0.084 & 0.735 $\pm$ 0.060 & 0.722 $\pm$ 0.049 \\
\bottomrule
\end{tabular}
\vspace{3pt}
\caption{\textbf{DS} help-detection on \textbf{Test=WEAK}. Transformer shows mean$\pm$std over folds; CP shows entropy and perplexity (mean$\pm$std across folds).}
\label{tab:ood_help_detection_test_weak}
\end{table*}

\subsection{Large In-Distribution Test Results}
Here we provide the detailed results of our large in-distribution test results.

\begin{table*}[h]
\centering
\small
\begin{tabular}{lcccc}
\toprule
Method & Acc. & Prec. & Rec. & F1 \\
\midrule
Strong Superv. & 0.802 $\pm$ 0.028 & 0.777 $\pm$ 0.024 & 0.695 $\pm$ 0.086 & 0.731 $\pm$ 0.050 \\
Weak Superv. & 0.656 $\pm$ 0.037 & 0.710 $\pm$ 0.098 & 0.217 $\pm$ 0.070 & 0.326 $\pm$ 0.085 \\
CP-S (entropy) & 0.499 $\pm$ 0.025 & 0.426 $\pm$ 0.029 & 0.801 $\pm$ 0.055 & 0.555 $\pm$ 0.030 \\
CP-S (perplex) & 0.490 $\pm$ 0.025 & 0.421 $\pm$ 0.029 & 0.805 $\pm$ 0.056 & 0.552 $\pm$ 0.029 \\
CP-W (entropy) & 0.497 $\pm$ 0.024 & 0.419 $\pm$ 0.025 & 0.733 $\pm$ 0.053 & 0.532 $\pm$ 0.025 \\
CP-W (perplex) & 0.479 $\pm$ 0.028 & 0.407 $\pm$ 0.030 & 0.715 $\pm$ 0.060 & 0.517 $\pm$ 0.034 \\
\bottomrule
\end{tabular}
\vspace{3pt}
\caption{Help detection on \textbf{Test=STRONG, L-ID} ($\beta=0.20$). Transformer shows mean$\pm$std over folds; CP shows entropy and perplexity (mean$\pm$std across folds).}
\label{tab:help_detection_test_strong_foldwise_lid}
\end{table*}

\begin{table*}[h]
\centering
\small
\begin{tabular}{lcccc}
\toprule
Method & Acc. & Prec. & Rec. & F1 \\
\midrule
Strong Superv. & 0.711 $\pm$ 0.048 & 0.679 $\pm$ 0.047 & 0.968 $\pm$ 0.027 & 0.797 $\pm$ 0.028 \\
Weak Superv. & 0.758 $\pm$ 0.082 & 0.797 $\pm$ 0.102 & 0.806 $\pm$ 0.089 & 0.796 $\pm$ 0.068 \\
CP-S (entropy) & 0.585 $\pm$ 0.036 & 0.585 $\pm$ 0.036 & 1.000 $\pm$ 0.000 & 0.738 $\pm$ 0.029 \\
CP-S (perplex) & 0.585 $\pm$ 0.036 & 0.585 $\pm$ 0.036 & 1.000 $\pm$ 0.000 & 0.738 $\pm$ 0.029 \\
CP-W (entropy) & 0.636 $\pm$ 0.063 & 0.656 $\pm$ 0.059 & 0.802 $\pm$ 0.070 & 0.720 $\pm$ 0.052 \\
CP-W (perplex) & 0.655 $\pm$ 0.034 & 0.670 $\pm$ 0.035 & 0.806 $\pm$ 0.053 & 0.731 $\pm$ 0.037 \\
\bottomrule
\end{tabular}
\vspace{3pt}
\caption{Help detection on \textbf{Test=WEAK, L-ID} ($\beta=0.20$). Transformer shows mean$\pm$std over folds; CP shows entropy and perplexity (mean$\pm$std across folds).}
\label{tab:help_detection_test_weak_foldwise_lid}
\end{table*}

\subsection{Sim OOD Test Results}
Here we provide the detailed results of our simulation out-of-distribution test results.

\begin{table*}[h]
\centering
\small
\begin{tabular}{l l cccc}
\toprule
Supervision & Variant & Acc. & Prec. & Rec. & F1 \\
\midrule
Weak Superv. & regular & 0.628 ± 0.058 & 0.760 ± 0.420 & 0.115 ± 0.073 & 0.196 ± 0.120 \\
Weak Superv. & jumbo & 0.722 ± 0.116 & 0.952 ± 0.110 & 0.370 ± 0.273 & 0.474 ± 0.268 \\
Weak Superv. & sim-only & 0.936 ± 0.044 & 0.938 ± 0.104 & 0.909 ± 0.069 & 0.918 ± 0.058 \\
Strong Superv. & regular & 0.738 ± 0.089 & 0.930 ± 0.132 & 0.386 ± 0.219 & 0.512 ± 0.233 \\
Strong Superv. & jumbo & 0.820 ± 0.057 & 0.848 ± 0.114 & 0.724 ± 0.226 & 0.748 ± 0.142 \\
\bottomrule
\end{tabular}
\caption{Sim-OOD (weak labels): Transformer variants comparison. Mean$\pm$std over folds.}
\label{tab:sim_weak_transformers}
\end{table*}
